Measurement of jet activity produced in top-quark events with an electron, a muon and two $b$-tagged jets in the final state in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

Measurements of jet activity in top-quark pair events produced in proton--proton collisions are presented, using 3.2 fb$^{-1}$ of $pp$ collision data at a centre-of-mass energy of 13 TeV collected by the ATLAS experiment at the Large Hadron Collider. Events are chosen by requiring an opposite-charge $e\mu$ pair and two $b$-tagged jets in the final state. The normalised differential cross-sections of top-quark pair production are presented as functions of additional-jet multiplicity and transverse momentum, $p_{\mathrm T}$. The fraction of signal events that do not contain additional jet activity in a given rapidity region, the gap fraction, is measured as a function of the $p_{\mathrm T}$ threshold for additional jets, and is also presented for different invariant mass regions of the $e\mu b\bar{b}$ system. All measurements are corrected for detector effects and presented as particle-level distributions compared to predictions with different theoretical approaches for QCD radiation. While the kinematics of the jets from top-quark decays are described well, the generators show differing levels of agreement with the measurements of observables that depend on the production of additional jets.

==> gaptablesystqsum.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|c|c|}
  \hline
  & \multicolumn{7}{c|}{Uncertainty in  $f_{\rm gap}(Q_{\mathrm{sum}})$ in [\%]}\\
  &  \multicolumn{7}{c|}{jet \pt\ threshold} \\
  & 25  & 45  & 65  & 110  & 150 & 250 & 380 \\
  Sources  &  \gev\ & \gev\ & \gev\ & \gev\ & \gev\ & \gev\ & \gev\ \\
  \hline \hline
Data statistics          & 1.2 & 0.9 & 0.7 & 0.5 & 0.4 & 0.3 & 0.2 \\
JES/JER             & 4.1 & 2.1 & 1.6 & 0.8 & 0.5 & 0.2 & 0.1 \\
b-tagging           & 0.5 & 0.4 & 0.3 & 0.2 & 0.1 & 0.1 & 0.0 \\
ISR/FSR Modelling   & 0.4 & 0.2 & 0.2 & 0.2 & 0.1 & 0.1 & 0.0 \\
Signal Modelling    & 4.5 & 2.0 & 1.3 & 0.9 & 0.8 & 0.6 & 0.3 \\
Other       & 1.1 & 0.5 & 0.4 & 0.3 & 0.2 & 0.1 & 0.1 \\ \hline
{\bf Total}               & {\bf 6.3} & {\bf 3.1} & {\bf 2.2} & {\bf 1.3} & {\bf 0.9} & {\bf 0.5} & {\bf 0.2} \\ \hline
\end{tabular}
\caption{Sources of uncertainty in the gap fraction measurement as a function of $Q_{\mathrm{sum}}$ for the full central region $|y|<2.1$, for a selection of $Q_{\mathrm{sum}}$ thresholds.}
\label{table:systqsum}
\end{table}

==> ratios.tex <==


\begin{figure}
\centering
\begin{tabular}{cc}
\subfloat[\label{fig:13a}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_feffVsNjets_emu25}}&
\subfloat[\label{fig:13b}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_feffVsNjets_emu40}}\\
\subfloat[\label{fig:13c}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_feff_Leadb_emu}}&
\subfloat[\label{fig:13d}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_feff_Leadadd_emu}}\\
\end{tabular}
\caption{  $ f_{\mathrm {eff}}$ as predicted by various MCs for (a)  jet multiplicity with jet \pt $>$ 25\,\gev, (b) jet multiplicity with jet \pt $>$ 40\,\gev, (c) leading \bjet\, \pt, (d)  leading additional jet \pt.
The uncertainties in the ratio plots represent the total uncertainties in the background predictions and statistical uncertainties in the signal. }
\label{fig:feff}
\end{figure}


\begin{figure}
\centering
\begin{tabular}{cc}
\subfloat[\label{fig:14a}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_faccVsNjets_emu25}}&
\subfloat[\label{fig:14b}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_faccVsNjets_emu40}}\\
\subfloat[\label{fig:14c}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_faccept_Leadb_emu}}&
\subfloat[\label{fig:14d}]{\includegraphics[width=0.5\textwidth]{figures/ttjets/unfoldingCorr_faccept_Leadadd_emu}}\\
\end{tabular}
\caption{  $ f_{\mathrm {accept}}$ as predicted by various MCs for (a)  jet multiplicity with jet \pt $>$ 25 \gev, (b) jet multiplicity with jet \pt $>$ 40 \gev, (c) leading \bjet\ \pt, (d)  leading additional jet \pt.
The uncertainties in the ratio plots represent the total uncertainties in the background predictions and statistical uncertainties in the signal. }
\label{fig:facc}
\end{figure}

\begin{figure}[ht]
\centering
\begin{tabular}{cc}
\subfloat[\label{fig:2a}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedNjets_PSRatios_emu25}}&
\subfloat[\label{fig:2b}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedNjets_PSRatios_emu40}}\\
\subfloat[\label{fig:2c}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedNjets_PSRatios_emu60}}&
\subfloat[\label{fig:2d}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedNjets_PSRatios_emu80}}\\
\end{tabular}
\caption{Ratios of jet multiplicity distribution for different \pt\ thresholds of the additional jets predicted by various parton shower generators to the unfolded data, for (a) additional jet \pt$>25$~\gev, (b) additional jet \pt$>40$~\gev, (c) additional jet \pt$>60$~\gev, and (d) additional jet \pt$>80$~\gev. The shaded regions show the statistical uncertainty (dark grey) and total uncertainty (light grey). 
\label{fig:multratiospsaux}}
\end{figure}


\begin{figure}[ht]
\centering
\begin{tabular}{cc}
\subfloat[\label{fig:2b}] {\includegraphics[width=0.45\textwidth]{figures/ttjets/unfoldedNjets_main_Ratios_emu40}}&
\subfloat[\label{fig:2d}] {\includegraphics[width=0.45\textwidth]{figures/ttjets/unfoldedNjets_main_Ratios_emu80}}\\
\end{tabular}
\caption{Ratios of unfolded jet multiplicity distribution for different \pt\ thresholds of the additional jets to various MC preditions.  Statistical errors (light gray) and total error (dark gray). 
 (a) additional jet \pt$>40$~\gev, (b) additional jet \pt$>80$\,\gev.
\label{fig:multratiosaux}}
\end{figure}

\clearpage


\begin{figure}[htbp]
\centering
\begin{tabular}{cc}
\subfloat[\label{fig:3a_1b}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedjetpt_Leadb_PSRatios_emu}} &
\subfloat[\label{fig:3b_1b}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedjetpt_Nleadb_PSRatios_emu}}
\end{tabular}
\begin{tabular}{c}
\subfloat[\label{fig:3ci_b}] {\includegraphics[width=0.42\textwidth]{figures/ttjets/unfoldedjetpt_Leadadd_PSRatios_emu} }
\end{tabular}
\caption{Ratios of jet \pt\ distribution for (a) leading $b$-jet, (b) sub-leading $b$-jet and (c) leading additional jet predicted by various MC generators to the unfolded data. \ The shaded regions show the statistical uncertainty (dark grey) and total uncertainty (light grey).
\label{fig:ptratiosaux}}
\end{figure}
\clearpage






==> simulation.tex <==



 Monte Carlo simulated event samples are used to develop the analysis, to compare to the data and to
evaluate signal and background efficiencies and uncertainties. Samples were processed either through
the full ATLAS detector simulation \cite{simul} based on GEANT4\cite{geant4}, or through a faster simulation making
use of parameterised showers in the calorimeters \cite{fastsim}. Additional simulated pp collisions generated with {\sc Pythia8.186} \cite{pythia8}  were overlaid to model the effects of both in- and out-of-time pileup, from additional pp
collisions in the same and nearby bunch crossings.  The pile-up distribution is reweighed to reflect the mean number of additional interactions observed in data. All simulated events were processed using the same
reconstruction algorithms and analysis chain as the data, and small corrections were applied to lepton
trigger and reconstruction efficiencies better to model the response observed in data.


 The baseline \ttbar\ full simulation sample was produced using
the next-to-leading-order (NLO) matrix element
generator {\sc Powheg-Box}~v2~\cite{powheg, powheg2,powheg3}
using the CT10 set of parton distribution functions \cite{cttenpdf},
and interfaced to
{\sc Pythia6.428}~\cite{pythia6} for the parton showering and fragmentation.
The Perugia 2012 (P2012)~\cite{perugia} parameter set (tune) with the CTEQ6L
PDF set \cite{ctsix} was used for the underlying event (UE) description.
All \ttbar\ final states involving at least one lepton are included.
The {\sc EvtGen} \cite{evtgen} package was used to model the decays of
heavy flavour hadrons.
The {\sc Powheg} model parameter hdampttt, which controls matrix element to
parton shower matching in {\sc Powheg} and effectively regulates the high-\pt 
radiation, was set to the top quark mass, 172.5~GeV, a setting which was found
to give the best modelling of the \ttbar system \pt  \cite{hdamp}.
The Standard Model expectation of $0.1082$  was
assumed for the $W\rightarrow\ell\nu$ branching ratio \cite{wbrpdg}.
%
Alternative \ttbar\, simulation samples were generated using {\sc Powheg}
interfaced to {\sc Herwig++} \cite{herwigpp}
 and {\sc MadGraph5\_aMC@NLO} \cite{amcnlo} interfaced to {\sc Herwig++}.
 The effects of initial- and final-state radiation (ISR/FSR) were explored using two alternative {\sc Powheg\,+\,Pythia6} samples,
 one with \hdampttt set to  $2\mtop$, the renormalisation scale set to half the
nominal value and using the Perugia 2012 radHi UE tune,
giving more radiation, and one with the Perugia 2012 radLo UE tune,
$\hdampttt=\mtop$ and the renormalisation scale set to twice the nominal value,
giving less radiation. These alternative \ttbar samples
were produced using fast simulation and compared to a fast simulation
version of the baseline sample.
The top quark mass was set to 172.5\,GeV in all the \ttbar simulation samples
mentioned above.

%
%  Background events are classified into two types: those with two real prompt
%leptons from $W$ or $Z$ decays (including those produced
%via leptonic tau decays), and those
%where at least one of the reconstructed lepton candidates is
%misidentified or `fake', {\em
%i.e.} a non-prompt lepton from the decay of a bottom or charm hadron,
%an electron from a photon conversion, hadronic jet activity misidentified
%as an electron, or a muon produced from an in-flight decay of a pion or
%kaon.
%%
%The first category with two prompt leptons includes $Wt$ single top production,
%$Z\rightarrow\tau\tau$+jets and dibosons ($WW$, $WZ$ and $ZZ$).
The backgrounds are simulated as follows:
$Wt$ production is modelled using {\sc Powheg-Box v2\,+\,Pythia6}
using the `diagram removal' generation scheme,
CT10 PDFs and the P2012 UE tune. An alternative calculation using the diagram subtraction scheme with  {\sc Powheg-Box v2\,+\,Pythia6}  was used  for the evaluation of the uncertainties on $Wt$. All  samples were normalised to the approximate NNLO cross-section of $71.7\pm3.8$\pb as determined in \cite{Kidonakis, arxiv:1005.4451}.


 $Z$  production including additional jets is modelled
for each decay channel separately ($ee$, $\mu\mu, \tau\tau$) using {\sc Sherpa} with CT10 PDFs.
%Inclusive $Z\rightarrow\tau\tau$ production
%(including additional jets) is modelled using {\sc Powheg} with CT10 PDFs,
%interfaced to
%{\sc Pythia8.186} and the AZNLO UE tune~\cite{aznlo} with CTEQ6L1 PDFs.
Diboson production in association with
jets is modelled using {\sc Sherpa} 2.1.1~\cite{sherpa} and CT10 PDFs,
including matrix elements calculated for up to one ($\ell\ell\nu\nu$ and
$\ell\ell\ell\ell$) or zero ($\ell\ell\ell\nu$) partons at NLO and up to
three partons at leading order using the {\sc Comix} \cite{comix}
and {\sc OpenLoops} \cite{openloops}
matrix element generators, merged with the {\sc Sherpa}
parton shower \cite{csshower}
using the ME+PS@NLO prescription \cite{mepsnlo}.

The majority of backgrounds with at least one misidentified lepton in the
selected sample arise from \ttbar production where only one of the top quarks
decays leptonically, which was simulated in the same way as dileptonic \ttbar
production.
%
Other backgrounds, including processes
with two misidentified leptons, are negligible
for the event selections used in this analysis.


 The object reconstruction, event selection and the application of calibration constants is performed using the common Top Group analysis software with the release versions
 AnalysisTop-2.3.45a and XRedTopAnalysis-00-06-21. The data derivation were produced with p2452, the MC derivations with p2516.


==> tables/results_jetpt.tex <==
\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
leading $b$-jet \pt\ [\gev] &  normalised cross-section for leading $b$-jet \pt\ \\
\hline
\hline
25-45 &  0.0027$\pm$0.0003$\pm$0.0005 \\  
45-65 &  0.0096$\pm$0.0005$\pm$0.0005 \\
65-85 &  0.0116$\pm$0.0005$\pm$0.0006 \\ 
85-110 &  0.0088$\pm$0.0004$\pm$0.0006 \\  
110-150 &  0.0044$\pm$0.0002$\pm$0.0003 \\  
150-250 &  0.0011$\pm$0.0001$\pm$0.0001 \\  
$>$ 250 &   0.000021$\pm$0.000002$\pm$0.000005 \\  
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the statistical and systematics uncertainties in terms of leading $b$-jet \pt.
\label{tab:resultsleadbjpt}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
next leading $b$-jet \pt\ [\gev] &  normalised cross-section for next leading $b$-jet \pt\ \\
\hline
\hline
25-40 &  0.0192$\pm$0.0008$\pm$0.0016 \\ 
40-55 &  0.0179$\pm$0.0007$\pm$0.0008 \\ 
55-75 &  0.0124$\pm$0.0005$\pm$0.0009 \\ 
75-100 &   0.0043$\pm$0.0003$\pm$0.0004 \\  
100-150 &  0.0014$\pm$0.0001$\pm$0.0001 \\ 
$>$ 150 &  0.000022$\pm$0.000002$\pm$0.000003 \\ 
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the statistical and systematics uncertainties in terms of next leading $b$-jet \pt.
\label{tab:resultsnleadbjpt}}
\end{center}
\end{table}


\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
leading-additional-jet \pt\ [\gev] &  normalised cross-section for leading-additional-jet \pt\ \\
\hline
\hline
25-40 &  0.0190$\pm$0.0007$\pm$0.0008 \\ 
40-60 &  0.0112$\pm$0.0006$\pm$0.0007 \\ 
60-85 &  0.0068$\pm$0.0004$\pm$0.0003  \\  
85-110 &  0.0040$\pm$0.0003$\pm$0.0004  \\ 
110-150 &  0.0021$\pm$0.0002$\pm$0.0002 \\  
150-250 &  0.0010$\pm$0.0001$\pm$0.0001 \\ 
$>$ 250 &  0.000058$\pm$0.000005$\pm$0.000004 \\  
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the statistical and systematics uncertainties in terms of leading-additional-jet \pt.
\label{tab:resultsleadaddjpt}}
\end{center}
\end{table}



\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|c|c|}
    \hline
 & 25--45~\gev & 45--65~\gev & 65--85~\gev & 85--110~\gev & 110--150~\gev & 150--250~\gev & $>$250~\gev \\
\hline
25-45~\gev & 1.0000 & - & - & - & - & - & - \\ 
45-65~\gev & 0.8727 & 1.0000 & - & - & - & - & - \\ 
65-85~\gev & -0.1761 & -0.1174 & 1.0000 & - & - & - & - \\ 
85-110~\gev & -0.8300 & -0.9037 & -0.0653 & 1.0000 & - & - & - \\ 
110-150~\gev & -0.8956 & -0.9127 & -0.0230 & 0.7990 & 1.0000 & - & - \\ 
150-250~\gev & -0.8446 & -0.9123 & -0.1122 & 0.8280 & 0.8539 & 1.0000 & - \\ 
$>$ 250~\gev & -0.7392 & -0.8196 & -0.0176 & 0.7297 & 0.7323 & 0.8064 & 1.0000 \\  
\hline
\end{tabular}
\caption{Correlation in total uncertainties across the leading $b$-jet \pt\ bins in the normalised differential cross-section measurement.
\label{tab:totUncCorleadb}}
\end{center}
\end{table}


\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
 & 25--40~\gev & 40--55~\gev & 55--75~\gev & 75--100~\gev & 100--150~\gev & $>$ 150~\gev \\ 
\hline
25-40~\gev & 1.0000 & - & - & - & - & - \\ 
40-55~\gev & 0.5723 & 1.0000 & - & - & - & - \\ 
55-75~\gev & -0.9271 & -0.7011 & 1.0000 & - & - & - \\ 
75-100~\gev & -0.9115 & -0.7251 & 0.8344 & 1.0000 & - & - \\ 
100-150~\gev & -0.9187 & -0.7421 & 0.8554 & 0.8811 & 1.0000 & - \\ 
$>$ 150~\gev & -0.8299 & -0.7393 & 0.8000 & 0.8106 & 0.8557 & 1.0000 \\ 
\hline
\end{tabular} 
\caption{Correlation in total uncertainties across the next to leading $b$-jet \pt\ bins in the normalised differential cross-section measurement.
\label{tab:totUncCornleadb}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|c|c|}
    \hline
  & 25--40~\gev & 40--60~\gev & 60--85~\gev & 85--110~\gev & 110--150~\gev & 150--250~\gev & $>$ 250~\gev \\ 
\hline
25-40~\gev & 1.0000 & - & - & - & - & - & - \\ 
40-60~\gev & 0.0643 & 1.0000 & - & - & - & - & - \\ 
60-85~\gev & -0.2214 & -0.4230 & 1.0000 & - & - & - & - \\ 
85-110~\gev & -0.1470 & -0.1566 & -0.2131 & 1.0000 & - & - & - \\ 
110-150~\gev & -0.6208 & -0.3892 & 0.0813 & -0.0871 & 1.0000 & - & - \\ 
150-250~\gev & -0.7898 & -0.3538 & 0.0970 & 0.0853 & 0.5545 & 1.0000 & - \\ 
$>$ 250~\gev & -0.6705 & -0.1779 & 0.0916 & 0.0349 & 0.3663 & 0.4692 & 1.0000 \\
\hline
\end{tabular} 
\caption{Correlation in total uncertainties across the leading-additional-jet \pt\ bins in the normalised differential cross-section measurement.
\label{tab:totUncCorleadadd}}
\end{center}
\end{table} 


==> tables/results_njets.tex <==
\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
additional-jet bin &  normalised cross-section for additional-jet $\pt>$25~\gev \\
\hline
\hline
0 &  0.4476$\pm$0.0092$\pm$0.0243 \\ 
1 &  0.3198$\pm$0.0085$\pm$0.0094 \\ 
2 &  0.1495$\pm$0.0060$\pm$0.0141 \\ 
3 &  0.0565$\pm$0.0036$\pm$0.0083 \\ 
$\ge$4 &  0.0267$\pm$0.0025$\pm$0.0058 \\ 
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the uncertainties in terms of additional-jet multiplicity measurements for additional jets with $\pt > 25$~\gev.
\label{tab:resultsnjets25}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
additional-jet bin &  normalised cross-section for additional-jet $\pt>$40~\gev \\
\hline
\hline
0 &  0.6068$\pm$0.0103$\pm$0.0180 \\ 
1 &  0.2781$\pm$0.0075$\pm$0.0128 \\ 
2 &  0.0885$\pm$0.0045$\pm$0.0072 \\ 
$\ge$3 &  0.0267$\pm$0.0024$\pm$0.0038 \\ 
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the uncertainties in terms of additional-jet multiplicity measurements for additional jets with $\pt > 40$~\gev. 
\label{tab:resultsnjets40}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|}
    \hline
additional-jet bin & normalised cross-section for additional-jet $\pt>$\,60~\gev \\
\hline
\hline
0 &  0.7305$\pm$0.0110$\pm$0.0101 \\ 
1 &  0.2144$\pm$0.0064$\pm$0.0069 \\ 
2 &  0.0450$\pm$0.0031$\pm$0.0034 \\ 
$\ge$3 &  0.0101$\pm$0.0015$\pm$0.0015 \\
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the uncertainties in terms of additional-jet multiplicity measurements for additional jets with $\pt > 60$~\gev.
\label{tab:resultsnjets60}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}  
\footnotesize
\begin{tabular}{|l|c|}
    \hline
additional-jet bin &  normalised cross-section for additional-jet $\pt>$80~\gev \\
\hline
\hline
0 &  0.8087$\pm$0.0115$\pm$0.0079 \\ 
1 &  0.1625$\pm$0.0054$\pm$0.0044 \\ 
2 &  0.0237$\pm$0.0023$\pm$0.0033 \\ 
$\ge$3 &  0.0051$\pm$0.0009$\pm$0.0016 \\
\hline
\end{tabular}
\caption{The measured normalised differential cross-section and the uncertainties in terms of additional-jet multiplicity measurements for additional jets with $\pt > 80$~\gev.
\label{tab:resultsnjets80}}
\end{center}
\end{table}



\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|}
    \hline
  & 0 & 1 & 2 & 3 & $\ge$4 \\
\hline
0 & 1.0000 & - & - & - & - \\ 
1 & -0.9116 & 1.0000 & - & - & - \\ 
2 & -0.8825 & 0.7477 & 1.0000 & - & - \\ 
3 & -0.7671 & 0.5670 & 0.5428 & 1.0000 & - \\ 
$\ge$4 & -0.4250 & 0.2271 & 0.1172 & 0.5593 & 1.0000 \\ 
\hline
\end{tabular}
\caption{Correlation in total uncertainties across the jet multiplicities in the normalised differential cross-section measurement for additional jets with $\pt > 25$~\gev.
\label{tab:totUncCornjets25}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|}
    \hline
  & 0 & 1 & 2 & $\ge$3 \\
\hline
0 & 1.0000 & - & - & - \\ 
1 & -0.9185 & 1.0000 & - & - \\ 
2 & -0.8671 & 0.6541 & 1.0000 & - \\ 
$\ge$3 & -0.4054 & 0.1132 & 0.3676 & 1.0000 \\ 
\hline
\end{tabular}
\caption{Correlation in total uncertainties across the jet multiplicities in the normalised differential cross-section measurement for additional jets with $\pt > 40$~\gev.
\label{tab:totUncCornjets40}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|}
    \hline
  & 0 & 1 & 2 & $\ge$3 \\
\hline
0 & 1.0000 & - & - & - \\ 
1 & -0.9527 & 1.0000 & - & - \\ 
2 & -0.8226 & 0.6256 & 1.0000 & - \\ 
$\ge$3 & 0.0154 & -0.2504 & 0.2454 & 1.0000 \\ 
\hline
\end{tabular}
\caption{Correlation in total uncertainties across the jet multiplicities in the normalised differential cross-section measurement for additional jets with $\pt > 60$~\gev.
\label{tab:totUncCornjets60}}
\end{center}
\end{table}


\begin{table}[ht!]
\begin{center}
\footnotesize
\begin{tabular}{|l|c|c|c|c|}
    \hline
  & 0 & 1 & 2 & $\ge$3 \\
\hline
0 & 1.0000 & - & - & - \\ 
1 & -0.9694 & 1.0000 & - & - \\ 
2 & -0.7708 & 0.6005 & 1.0000 & - \\ 
$\ge$3 & 0.1322 & -0.3029 & 0.1708 & 1.0000 \\ 
\hline
\end{tabular}
\caption{Correlation in total uncertainties across the jet multiplicities in the normalised differential cross-section measurement for additional jets with $\pt > 80$~\gev.
\label{tab:totUncCornjets80}}
\end{center}
\end{table} 

